Hybridizing Non-dominated Sorting Algorithms: Divide-and-Conquer Meets Best Order Sort

Many production-grade algorithms benefit from combining an asymptotically efficient algorithm for solving big problem instances, by splitting them into smaller ones, and an asymptotically inefficient algorithm with a very small implementation constant for solving small subproblems. A well-known example is stable sorting, where mergesort is often combined with insertion sort to achieve a constant but noticeable speed-up. We apply this idea to non-dominated sorting. Namely, we combine the divide-and-conquer algorithm, which has the currently best known asymptotic runtime of $O(N (\log N)^{M - 1})$, with the Best Order Sort algorithm, which has the runtime of $O(N^2 M)$ but demonstrates the best practical performance out of quadratic algorithms. Empirical evaluation shows that the hybrid's running time is typically not worse than of both original algorithms, while for large numbers of points it outperforms them by at least 20%. For smaller numbers of objectives, the speedup can be as large as four times.

==> parts/nds-common.tex <==
\newcommand{\NDSIntroduction}{
Many real-world optimization problems are multiobjective, that is, they require maximizing or
minimizing several objectives, which are often conflicting. These problems most often do not have
a single solution, but instead feature many incomparable solutions, which trade one objective for another.
It is often not known \emph{a priori} which solution will be chosen, as decisions of this sort
are often recommended to be made late, as the decision maker can learn more about the problem~\cite{gecco-2016-emo-tutorial}.
This encourages finding a set of diverse incomparable solutions,
which is a problem often approached by multiobjective evolutionary algorithms.

In the realm of scaling-independent preference-less, and thus general-purpose, evolutionary multiobjective algorithms,
three paradigms currently seem to prevail~\cite{gecco-2016-emo-tutorial}:
Pareto-based, indicator-based, and decomposition-based approaches.
Although there exist well-known decomposition-based~\cite{moea-d} and indicator-based~\cite{hypervolume,ibea,epsilon-indicator} algorithms,
the majority of modern algorithms are Pareto-based~\cite{nsga-ii,nsga-iii,pesa-ii,spea2}.

Most Pareto-based algorithms belong to one of big groups according to how solutions are selected or ranked:
the algorithms which maintain non-dominated solutions~\cite{pesa-ii,paes,micro-ga},
perform non-dominated sorting~\cite{nsga-ii,nsga-iii,npga2}, use domination count~\cite{fonseca-moga}, or domination strength~\cite{spea2}.
In this research we concentrate on non-dominated sorting, as some popular algorithms make use of it~\cite{nsga-ii,nsga-iii}.

Non-dominated sorting assigns ranks to solutions in the following way: the non-dominated solutions get rank 0,
and the solutions which are dominated only by solutions of rank at most $i$ get rank $i+1$. In the original work~\cite{nsga},
this procedure was performed in $O(N^3 M)$, where $N$ is the population size and $M$ is the number of objectives. This was later improved
to be $O(N^2 M)$ in~\cite{nsga-ii}.

As the quadratic complexity is still quite large, both from theoretical and practical points of view,
many researchers concentrated on improving practical running times~\cite{zhang-ens,zhang-ens-presort,fang-nds-tree,gustavsson-nds,best-order-sort-gecco,deductive-climbing-sort,corner-sort},
however, without improving the worst-case $O(N^2 M)$ complexity. Jensen was the first to adapt the earlier result of Kung et at.~\cite{kung75},
who solved the problem of finding non-dominated solutions in $O(N (\log N)^{\max(1, M-2)})$, to non-dominated sorting.
This algorithm has the worst-case complexity of $O(N (\log N)^{M-1})$. However, this algorithm could not handle coinciding objective values,
which was later corrected in subsequent works~\cite{fortin,buzdalov-nds-2014}. A more efficient algorithm for non-dominated sorting,
or finding \emph{layers of maxima}, exists for three dimensions~\cite{nekrich-fast-3d-nds}, whose complexity is
$O(N (\log \log N)^2)$ with the use of randomized data structures, or $O(N (\log \log N)^3)$ for deterministic ones.
However, whether this algorithm is useful in practice is still an open question.
}

\newcommand{\NDSPreliminariesSet}{
In the following, we assume that all points are different, which enables us to name any unordered collection of points a \emph{set}.
This is not true in general, however, all equal points will receive the same rank, so implementations are free, depending on their need,
to either discard a point if there is an equal one, or to keep all equal points in a same entity and run algorithms on these entities instead,
or to work directly with equal points with some additional algorithmic care. None of these precautions change the worst-case algorithmic complexity.
}

\newcommand{\NDSPreliminariesLetters}{
We use capital Latin letters to denote sets of points, as well as the global constants $N$ (the 
number of points) and $M$ (the number of objectives),
while small Latin letters are used for single points, standalone objectives and rank values,
and small Greek letters are used for mappings. The value of the $i$-th objective of a point $p$ is 
denoted as $p_i$.
}

\newcommand{\NDSPreliminariesPareto}{
In the rest of the paper we assume, without losing generality, that we solve a multiobjective minimization problem
with the number of objectives equal to $M$.
In this case, the \emph{Pareto dominance relation} is determined on two points in the objective space as follows:
\begin{align*}
    a \prec b   &\leftrightarrow \forall i \in [1; M] \; a_i \le b_i
                    \text{ and } \exists i \in [1; M] \; a_i < b_i \\
    a \preceq b &\leftrightarrow \forall i \in [1; M] \; a_i \le b_i
\end{align*}
where $a \prec b$ is called the \emph{strict dominance} and $a \preceq b$ is the \emph{weak dominance}.
}

\newcommand{\NDSPreliminariesOfflineNDS}{
\emph{Non-dominated sorting} is a procedure which, for a given set $P$ of $N$ points in the $M$-dimensional objective space,
assigns each point $p \in P$ an integer \emph{rank} $\tau(p)$, such that:
\begin{align*}
\tau(p) = \max \{0\} \cup \{ 1 + \tau(q) \mid q \in P, q \prec p \}.
\end{align*}
In other words, a rank of a point which is not dominated by any other point is zero,
and a rank of any other point is one plus the maximum rank among the points which dominate it.

Following the convention from~\cite{deb-enlu-14},
we call the set of all points with the given rank $r$ a \emph{non-domination level} $L_r$:
\begin{align*}
L_r = \{ p \in P \mid \tau(p) = r \}.
\end{align*}
}

\newcommand{\NDSDivideAndConquer}{
The divide-and-conquer approach dates back to 1975, when Kung et al. proposed a multidimensional divide-and-conquer algorithm
for finding the maxima of a set of vectors~\cite{kung75}, which, in the realm of evolutionary computation,
corresponds to the set of non-dominated points, or to points with rank zero.
The complexity of this algorithm is $O(\min(N^2, N (\log N)^{\max(1, M - 2)})))$,
which we shorten to $O(N (\log N)^{M - 2})$ for clarity.

This algorithm can be used to implement non-dominated sorting in the following manner: first we determine the points with rank zero,
then we remove these points and run the algorithm again on the remaining points (which yields points with rank one),
then we repeat it until no points left. However, the worst-case complexity of this approach is $O(N^2 (\log N)^{M - 2})$.
In contrast, fast non-dominated sorting, shipped with the original NSGA-II of Deb et at.~\cite{nsga-ii}, has a better $O(N^2 M)$ complexity.

The divide-and-conquer approach has been generalized to perform non-dominated sorting by Jensen~\cite{jensen},
shortly afterwards the NSGA-II arrived. The algorithm from~\cite{jensen} solves the problem in $O(N (\log N)^{M - 1})$,
which is much faster for small values of $K$, as well as for large values of $N$, than fast non-dominated sorting.
However, this algorithm was designed with an assumption that no two points have equal objectives, which is often not the case,
especially in discrete optimization, and is known to produce wrong results when this assumption is violated.
This problem was overcome by Fortin et al.~\cite{fortin}, who proposed modifications of this algorithm to always produce
correct results. The average complexity was proven to be the same, but the worst-case complexity was left at $O(N^2 M)$.
Finally, Buzdalov et al.~\cite{buzdalov-nds-2014} introduced further modifications to achieve the worst-case
time complexity of $O(N (\log N)^{M - 1})$.

We shall now briefly illustrate the working principles of this approach. At any moment of time,
the algorithm maintains, for every point $p$, a lower bound on its rank $r'(p)$, which are initially
set to zero. The reason for this lower bound can be explained as follows: at any moment of time,
we have performed a subset of necessary objective comparisons, which impose approximations of ranks
of the affected points. These approximations are of course lower bounds of the real ranks.

To ease the notation, in the following we do not use the term ``lower bound of the rank'', as well as the $r'$ symbol.
Instead, we will say ``current rank'' for the current state of the lower bound of a certain point, which possibly
coincides with the real rank, and ``final rank'' when we know that the lower bound coincides with the real rank.

One of the main properties of the algorithm is that whenever a comparison of $p_m$ and $q_m$ is performed for the first time,
where $p$ and $q$ are points and $1 \le m \le M$ is the objective, then the following holds:
\begin{itemize}
    \item for all objectives $m'$ such that $m < m' \le M$, it holds that $p_{m'} \le q_{m'}$, that is,
          $p$ weakly dominates $q$ in objectives $[m';M]$;
    \item the rank of $p$ is known and final, that is, all comparisons necessary to determine the rank of $p$
          have already been done.
\end{itemize}

The top-level concept is the procedure $\textsc{HelperA}(S, m)$, which takes a set of points $S$ sorted lexicographically
(where non-zero lower bounds are possibly known for some of the points from $S$)
and makes sure all necessary comparisons between the objectives $[1;m]$ of these points are performed.
This procedure is called only when all necessary comparisons of points $p$ and $q$, such that $q \in S$ and $p \notin S$,
have already been performed.
To perform non-dominated sorting of a set $P$ with $M$ objectives, one should run $\textsc{HelperA}(P, M)$.

For $m = 2$, it calls a sweep line based algorithm $\textsc{SweepA}(S)$, which runs in $O(|S| \log |S|)$, which we will cover later.
If there are at most two points in $S$, it performs their direct comparisons and updates the rank of the
second point if necessary. If all values of the objective $m$ are the same in the entire $S$,
it directly calls $\textsc{HelperA}(S, m - 1)$.
Otherwise, it divides $S$ into three parts using the objective $m$:
the $S_L$ part with lower values, the $S_M$ part with median values,
and the $S_H$ part with higher values.

It is clear that ranks of points in $S_L$ do not depend on ranks of points in neither $S_M$ nor $S_H$,
and $S_M$ also does not depend on $S_H$. The algorithm first calls $\textsc{HelperA}(S_L, m)$,
which results in finding the exact ranks in $S_L$, because all necessary comparisons with points from $S_L$ on the right side
and other points on the left side have been performed before this call.

Next comes the set $S_M$, but the ranks of these points still need to be updated using the set $S_L$ (and nothing more).
To do this, the algorithm calls another procedure, $\textsc{HelperB}(S_L, S_M, m - 1)$, whose meaning is to update
the ranks of points from the second argument using the first argument and objectives in $[1; m-1]$.
Then it calls $\textsc{HelperA}(S_M, m - 1)$, as all other necessary comparisons have been done, and all values for the objective $m$
are equal in $S_M$. It then proceeds with $\textsc{HelperB}(S_L \cup S_M, S_H, m - 1)$ and finishes with $\textsc{HelperA}(S_H, m)$.

The $\textsc{HelperB}(L, H, m)$ procedure, as follows from the short description above, shall perform all the necessary comparisons
between points $p \in L$ on the left and $q \in H$ on the right, provided that in objectives $[m+1; M]$ it holds that $p \prec q$,
and all ranks in $L$ are final. For $m = 2$, it, again, runs a sweep line procedure $\textsc{SweepB}(L, H)$.
If $|L| = 1$ or $|H| = 1$, a straightforward pairwise comparison is performed. If the maximum value of the objective $m$ in $L$
does not exceed the minimum value in $H$, it calls $\textsc{HelperB}(L, H, m-1)$. Otherwise, it chooses a median of the objective $m$
in $L \cup H$ and then, similarly to \textsc{HelperA}, splits $L$ into $L_L$, $L_M$ and $L_H$,
and also splits $H$ into $H_L$, $H_M$ and $H_H$. Following the same logic as in \textsc{HelperA}, it performs the following
recursive calls:
\begin{itemize}
    \item $\textsc{HelperB}(L_L, H_L, m)$;
    \item $\textsc{HelperB}(L_L, H_M, m - 1)$;
    \item $\textsc{HelperB}(L_M, H_M, m - 1)$;
    \item $\textsc{HelperB}(L_L \cup L_M, H_H, m - 1)$;
    \item $\textsc{HelperB}(L_H, H_H, m)$.
\end{itemize}

\begin{figure*}[!t]
\begin{tikzpicture}[scale=0.38]
\TikZPictureSweepA
\end{tikzpicture}
\caption{Example iterations of the \textsc{SweepA} procedure.
Gray points are those whose rank is determined, the darker ones
constitute a binary search tree and thus connected with dotted lines.
The numbers in white points are the lower bounds on ranks.
The vertical dashed line is the sweep line.
In (b), the representer of level 2 is removed as all possible remaining
points dominated by that point are also dominated by the representer of level 3;
similar thing happens in (c).
}\label{sweep-a-example}
\end{figure*}

The remaining parts to explain are $\textsc{SweepA}(S)$ and $\textsc{SweepB}(L, H)$.
The \textsc{SweepA} procedure utilizes a sweep line approach. Points from the set $S$
are processed in lexicographical order using first two objectives. In the same time,
the procedure maintains a binary search tree which contains the last seen representative points
for each non-domination level. When the next point is processed, this binary search tree is traversed
to determine the biggest number of the level which still dominates the point in question, and then
the rank of this point is updated correspondingly. After that, this point is inserted in the tree:
it becomes the last representative of its non-domination level and possibly throws out some of
the other representatives, which have no more chance to determine rank of any point on their own.
An example is shown in Fig.~\ref{sweep-a-example}.

The \textsc{SweepB} procedure works in a similar way. The sweep line goes over the union of sets, $L \cup H$,
however, the tree is built of the points from $L$ only, and rank updates are performed with points from $H$ only.

The running times of \textsc{SweepA} and \textsc{SweepB} are $O(|S| \log |S|)$ and $O((|L| + |H|) \log |L|)$,
respectively. From the well-known theory of solving recursive relations, and from the strategies of creating subproblems,
it follows that the running time of $\textsc{HelperB}(L, H, m)$ is $O((|L| + |H|) \cdot (\log (|L| + |H|))^{m - 1})$,
and of $\textsc{HelperA}(S, m)$ it is $O(|S| \cdot (\log |S|)^{m - 1})$.
}

